An Automata Theoretic Approach to the Zero-One Law for Regular Languages: Algorithmic and Logical Aspects

A zero-one language L is a regular language whose asymptotic probability converges to either zero or one. In this case, we say that L obeys the zero-one law. We prove that a regular language obeys the zero-one law if and only if its syntactic monoid has a zero element, by means of Eilenberg's variety theoretic approach. Our proof gives an effective automata characterisation of the zero-one law for regular languages, and it leads to a linear time algorithm for testing whether a given regular language is zero-one. In addition, we discuss the logical aspects of the zero-one law for regular languages.

==> eptcsdata.tex <==
\providecommand{\firstpage}{172}
\providecommand{\publicationstatus}{J. Esparza, E. Tronci (Eds.): Games, Automata,\\ 
Logics and Formal Verification 2015 (GandALF'15)\\
EPTCS 193, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.193.13}{10.4204/EPTCS.193.13}}
\pdfoutput=1

